A search for top squarks with R-parity-violating decays to all-hadronic final states with the ATLAS detector in $\sqrt{s}$ = 8 TeV proton-proton collisions

A search for the pair production of top squarks, each with R-parity-violating decays into two Standard Model quarks, is performed using 17.4 fb$^{-1}$ of $\sqrt{s}$ = 8 TeV proton-proton collision data recorded by the ATLAS experiment at the LHC. Each top squark is assumed to decay to a b- and an s-quark, leading to four quarks in the final state. Background discrimination is achieved with the use of b-tagging and selections on the mass and substructure of large-radius jets, providing sensitivity to top squark masses as low as 100 GeV. No evidence of an excess beyond the Standard Model background prediction is observed and top squarks decaying to $\bar{b}\bar{s}$ are excluded for top squark masses in the range $100 \leq m_{\tilde{t}} \leq 315$ GeV at 95% confidence level.

==> tab-CLs.tex <==
%%------------------------------  
\begin{table}[!ht]
\begin{center}\renewcommand\arraystretch{1.6}
\sisetup{
scientific-notation=true,
detect-mode,
tight-spacing           = true,
input-open-uncertainty  = ,
input-close-uncertainty = ,
round-mode              = figures,
round-precision         = 2,
table-space-text-pre    = ( [,
table-space-text-post   = ) ] \Star, 
}
\begin{tabular}{c| S[table-text-alignment=center] S[table-text-alignment=center]}
\toprule
{$m_{\tilde{t}}\,[{\rm GeV}]$} & {Observed $CLs$} & {Expected $CLs$} \\
\midrule
100 & 2.808890e-06 & 1.160986e-05 \\
125 & 8.156165e-06 & 1.114104e-05 \\
150 & 9.065742e-06 & 1.954338e-05 \\
175 & 1.072044e-03 & 1.902746e-04 \\
200 & 5.534995e-05 & 4.431543e-05 \\
225 & 1.871313e-03 & 8.900281e-04 \\
250 & 7.483455e-03 & 2.590600e-03 \\
275 & 4.818216e-03 & 9.330888e-03 \\
300 & 2.995775e-03 & 1.739485e-02 \\
325 & 7.874563e-02 & 7.520543e-02 \\
350 & 2.773246e-01 & 1.037727e-01 \\
375 & 3.304040e-01 & 2.605206e-01 \\
400 & 1.809102e-01 & 2.646336e-01 \\
\bottomrule          
\end{tabular}
\caption{Observed and expected $95\%$ $CLs$ for the stop signal samples.}
\label{tab:aux-CLs}
\end{center}
\end{table}
%%------------------------------  


==> tab-contamination-signal.tex <==
\begin{table}[!ht]
\tiny
\begin{center}\renewcommand\arraystretch{1.6}
\sisetup{round-mode=figures, round-precision=2,
retain-explicit-plus=true, group-digits = true}
\scalebox{0.9}{
\begin{tabular}{c|c|
l|l|l|l|l|l|l|l|l|l|l|l}
\toprule
$m_{\tilde{t}}[{\rm GeV}]$ & {Window [${\rm GeV}$]} & {$N_{A0}$} & {$N_{B0}$} & {$N_{C0}$} & {$N_{D0}$} & {$N_{A1}$} & {$N_{B1}$} & {$N_{C1}$} & {$N_{D1}$} & {$N_{A2}$} & {$N_{B2}$} & {$N_{C2}$} & {$N_{D2}$} \\
\midrule
100 & [95, 115] & $0.21\,\%$ & $0.64\,\%$ & $0.42\,\%$ & $4\,\%$ & $1.2\,\%$ & $14\,\%$ & $4.8\,\%$ & $29\,\%$ & $2.2\,\%$ & $50\,\%$ & $8.2\,\%$ & $120\,\%$ \\
125 & [115, 135] & $0.069\,\%$ & $1.4\,\%$ & $0.16\,\%$ & $3\,\%$ & $0.64\,\%$ & $13\,\%$ & $2.5\,\%$ & $30\,\%$ & $3.1\,\%$ & $43\,\%$ & $7.1\,\%$ & $100\,\%$ \\
150 & [135, 165] & $0.048\,\%$ & $0.9\,\%$ & $0.088\,\%$ & $2\,\%$ & $0.46\,\%$ & $9.7\,\%$ & $1.6\,\%$ & $31\,\%$ & $1.7\,\%$ & $29\,\%$ & $4.1\,\%$ & $73\,\%$ \\
175 & [165, 190] & $0.019\,\%$ & $0.5\,\%$ & $0.02\,\%$ & $2.3\,\%$ & $0.48\,\%$ & $8\,\%$ & $1.3\,\%$ & $21\,\%$ & $1.2\,\%$ & $24\,\%$ & $2.8\,\%$ & $72\,\%$ \\
200 & [185, 210] & $0.056\,\%$ & $0.49\,\%$ & $0.21\,\%$ & $2.3\,\%$ & $0.39\,\%$ & $8.2\,\%$ & $1.2\,\%$ & $26\,\%$ & $1.4\,\%$ & $23\,\%$ & $3.9\,\%$ & $71\,\%$ \\
225 & [210, 235] & $0.034\,\%$ & $0.48\,\%$ & $0.14\,\%$ & $2.1\,\%$ & $0.57\,\%$ & $8\,\%$ & $0.91\,\%$ & $22\,\%$ & $1.6\,\%$ & $28\,\%$ & $2.7\,\%$ & $63\,\%$ \\
250 & [235, 265] & $0.075\,\%$ & $0.47\,\%$ & $0.11\,\%$ & $2.2\,\%$ & $0.54\,\%$ & $6.3\,\%$ & $0.94\,\%$ & $20\,\%$ & $1.7\,\%$ & $25\,\%$ & $2\,\%$ & $65\,\%$ \\
275 & [260, 295] & $0.089\,\%$ & $0.4\,\%$ & $0\,\%$ & $2\,\%$ & $0.58\,\%$ & $7.4\,\%$ & $1.6\,\%$ & $20\,\%$ & $1.6\,\%$ & $23\,\%$ & $2.2\,\%$ & $74\,\%$ \\
300 & [280, 315] & $0.031\,\%$ & $0.69\,\%$ & $0.098\,\%$ & $2.5\,\%$ & $0.23\,\%$ & $8.8\,\%$ & $1.1\,\%$ & $26\,\%$ & $1.6\,\%$ & $31\,\%$ & $0.64\,\%$ & $94\,\%$ \\
325 & [305, 350] & $0\,\%$ & $0.87\,\%$ & $0.077\,\%$ & $1.8\,\%$ & $0.67\,\%$ & $9.5\,\%$ & $1.6\,\%$ & $25\,\%$ & $1.8\,\%$ & $25\,\%$ & $5.2\,\%$ & $67\,\%$ \\
350 & [325, 370] & $0.029\,\%$ & $0.64\,\%$ & $0.13\,\%$ & $2.1\,\%$ & $0.71\,\%$ & $7\,\%$ & $1.7\,\%$ & $18\,\%$ & $1.3\,\%$ & $31\,\%$ & $2.8\,\%$ & $55\,\%$ \\
375 & [345, 395] & $0.085\,\%$ & $0.95\,\%$ & $0.21\,\%$ & $3.4\,\%$ & $0.49\,\%$ & $7.7\,\%$ & $0.63\,\%$ & $18\,\%$ & $1.8\,\%$ & $26\,\%$ & $6.2\,\%$ & $57\,\%$ \\
400 & [375, 420] & $0.11\,\%$ & $0.68\,\%$ & $0.24\,\%$ & $2.4\,\%$ & $0.22\,\%$ & $10\,\%$ & $0.28\,\%$ & $43\,\%$ & $1\,\%$ & $26\,\%$ & $2.8\,\%$ & $160\,\%$ \\
\bottomrule
\end{tabular}
}
\caption{Breakdown of expected signal contribution ($N_S/N_{\rm data}$) for all sidebands and mass windows. All numbers are shown as percentages.}
\label{tab:contamination:signal}
\end{center}
\end{table}


==> tab-contamination-ttbar.tex <==
\begin{table}[!ht]
\tiny
\begin{center}\renewcommand\arraystretch{1.6}
\sisetup{round-mode=figures, round-precision=2,
retain-explicit-plus=true, group-digits = true}
\scalebox{0.9}{
\begin{tabular}{c|c|
l|l|l|l|l|l|l|l|l|l|l}
\toprule
{Window [${\rm GeV}$]} & {$N_{A0}$} & {$N_{B0}$} & {$N_{C0}$} & {$N_{D0}$} & {$N_{A1}$} & {$N_{B1}$} & {$N_{C1}$} & {$N_{D1}$} & {$N_{A2}$} & {$N_{B2}$} & {$N_{C2}$} & {$N_{D2}$} \\
\midrule
$[95, 115]$ & $0.27\,\%$ & $0.2\,\%$& $0.39\,\%$ & $0.27\,\%$ & $2.6\,\%$ & $1.9\,\%$ & $3.4\,\%$ & $2.3\,\%$ & $6.8\,\%$ & $7.2\,\%$ & $8.8\,\%$ & $8.4\,\%$ \\
$[115, 135]$ & $0.22\,\%$ & $0.16\,\%$& $0.35\,\%$ & $0.25\,\%$ & $2.3\,\%$ & $2.1\,\%$ & $3.4\,\%$ & $2.9\,\%$ & $7.3\,\%$ & $9.5\,\%$ & $9.9\,\%$ & $12\,\%$ \\
$[135, 165]$ & $0.14\,\%$ & $0.17\,\%$& $0.2\,\%$ & $0.29\,\%$ & $1.5\,\%$ & $2.3\,\%$ & $2.1\,\%$ & $3.6\,\%$ & $5.7\,\%$ & $10\,\%$ & $7.5\,\%$ & $14\,\%$ \\
$[165, 190]$ & $0.072\,\%$ & $0.14\,\%$& $0.093\,\%$ & $0.24\,\%$ & $0.74\,\%$ & $1.9\,\%$ & $0.99\,\%$ & $3.7\,\%$ & $2.8\,\%$ & $8.8\,\%$ & $2.9\,\%$ & $11\,\%$ \\
$[185, 210]$ & $0.057\,\%$ & $0.052\,\%$& $0.072\,\%$ & $0.089\,\%$ & $0.69\,\%$ & $0.72\,\%$ & $0.93\,\%$ & $1\,\%$ & $2.2\,\%$ & $2.4\,\%$ & $3.1\,\%$ & $4\,\%$ \\
$[210, 235]$ & $0.056\,\%$ & $0.029\,\%$& $0.1\,\%$ & $0.035\,\%$ & $0.72\,\%$ & $0.29\,\%$ & $1.1\,\%$ & $0.24\,\%$ & $2.4\,\%$ & $0.8\,\%$ & $2.6\,\%$ & $0.85\,\%$ \\
$[235, 265]$ & $0.038\,\%$ & $0.014\,\%$& $0.097\,\%$ & $0.032\,\%$ & $0.65\,\%$ & $0.2\,\%$ & $1\,\%$ & $0.36\,\%$ & $2\,\%$ & $0.61\,\%$ & $2.5\,\%$ & $0.56\,\%$ \\
$[260, 295]$ & $0.061\,\%$ & $0.029\,\%$& $0.06\,\%$ & $0.031\,\%$ & $0.61\,\%$ & $0.25\,\%$ & $1.1\,\%$ & $0.3\,\%$ & $1.9\,\%$ & $0.53\,\%$ & $2.2\,\%$ & $0.62\,\%$ \\
$[280, 315]$ & $0.11\,\%$ & $0.024\,\%$& $0.071\,\%$ & $0.047\,\%$ & $0.61\,\%$ & $0.18\,\%$ & $0.99\,\%$ & $0.32\,\%$ & $2.3\,\%$ & $0.86\,\%$ & $2.9\,\%$ & $1.8\,\%$ \\
$[305, 350]$ & $0.085\,\%$ & $0.017\,\%$& $0.17\,\%$ & $0\,\%$ & $0.77\,\%$ & $0.19\,\%$ & $0.87\,\%$ & $0.3\,\%$ & $1.8\,\%$ & $0.66\,\%$ & $3.5\,\%$ & $1.7\,\%$ \\
$[325, 370]$ & $0.13\,\%$ & $0.065\,\%$& $0.14\,\%$ & $0\,\%$ & $0.73\,\%$ & $0.35\,\%$ & $0.76\,\%$ & $0.28\,\%$ & $1.9\,\%$ & $0.72\,\%$ & $3.5\,\%$ & $0.62\,\%$ \\
$[345, 395]$ & $0.13\,\%$ & $0.15\,\%$& $0.19\,\%$ & $0\,\%$ & $0.7\,\%$ & $0.29\,\%$ & $0.88\,\%$ & $0.26\,\%$ & $1.9\,\%$ & $0.82\,\%$ & $4.3\,\%$ & $0.35\,\%$ \\
$[375, 420]$ & $0.037\,\%$ & $0.13\,\%$& $0.18\,\%$ & $0\,\%$ & $0.71\,\%$ & $0.089\,\%$ & $0.76\,\%$ & $0.0001\,\%$ & $1.9\,\%$ & $0.24\,\%$ & $2.7\,\%$ & $0.51\,\%$ \\
\bottomrule
\end{tabular}
}
\caption{Breakdown of \ttbar \ contribution ($N_{\ttbar}/N_{\rm data}$) for all sidebands and mass windows. All numbers are shown as percentages.}
\label{tab:contamination:ttbar}
\end{center}
\end{table}


==> tab-syst-signal.tex <==
\begin{table}[!ht]
\scriptsize
\begin{center}\renewcommand\arraystretch{1.6}
\sisetup{round-mode=figures, round-precision=2,
retain-explicit-plus=true, group-digits = true}
\begin{tabular}{
c|c|
S[table-format=3.1, table-number-alignment=center, round-mode=figures, round-precision=2] | 
S[table-format=4.2, table-number-alignment=center, round-mode=figures, round-precision=2] | 
c|
S[table-format=4.3, table-number-alignment=center, round-mode=figures, round-precision=2] | 
c|c|c}
\toprule
$m_{\tilde{t}}\,[{\rm GeV}]$ & {Window [${\rm GeV}$]} & {$N_S$} & {Statistics} & {JES} & {JER} & {$b$-tag} & {Theory} & {Total uncertainty} \\
\midrule
100 & [95, 115] & 562.86 & {$\pm$}62.54 & \numpmRF{+102.28}{-64.74}{2} & {$\pm$}20.44 & \numpmRF{+73.14}{-68.84}{2} & \numpmRF{+25.41}{-23.86}{2} & \numpmRF{+144.17}{-117.60}{2} \\
125 & [115, 135] & 570.86 & {$\pm$}46.15 & \numpmRF{+65.55}{-34.57}{2} & {$\pm$}65.33 & \numpmRF{+70.61}{-66.72}{2} & \numpmRF{+22.97}{-24.01}{2} & \numpmRF{+127.32}{-112.35}{2} \\
150 & [135, 165] & 557.13 & {$\pm$}34.29 & \numpmRF{+71.09}{-48.87}{2} & {$\pm$}27.57 & \numpmRF{+69.11}{-65.01}{2} & \numpmRF{+24.97}{-26.97}{2} & \numpmRF{+111.31}{-96.32}{2} \\
175 & [165, 190] & 421.02 & {$\pm$}28.51 & \numpmRF{+13.84}{-68.75}{2} & {$\pm$}26.79 & \numpmRF{+54.15}{-50.88}{2} & \numpmRF{+21.45}{-20.29}{2} & \numpmRF{+71.52}{-96.21}{2} \\
200 & [185, 210] & 293.46 & {$\pm$}17.57 & \numpmRF{+23.30}{-27.97}{2} & {$\pm$}2.18 & \numpmRF{+36.74}{-34.63}{2} & \numpmRF{+15.15}{-14.29}{2} & \numpmRF{+49.35}{-49.99}{2} \\
225 & [210, 235] & 177.67 & {$\pm$}9.96 & \numpmRF{+10.80}{-23.49}{2} & {$\pm$}3.56 & \numpmRF{+24.20}{-22.63}{2} & \numpmRF{+9.76}{-9.32}{2} & \numpmRF{+30.16}{-35.54}{2} \\
250 & [235, 265] & 126.84 & {$\pm$}6.48 & \numpmRF{+8.60}{-22.50}{2} & {$\pm$}2.78 & \numpmRF{+17.08}{-16.05}{2} & \numpmRF{+7.78}{-7.03}{2} & \numpmRF{+21.81}{-29.38}{2} \\
275 & [260, 295] & 71.31 & {$\pm$}6.74 & \numpmRF{+6.67}{-12.82}{2} & {$\pm$}8.75 & \numpmRF{+10.86}{-10.10}{2} & \numpmRF{+5.95}{-4.67}{2} & \numpmRF{+17.88}{-20.25}{2} \\
300 & [280, 315] & 48.19 & {$\pm$}4.28 & \numpmRF{+1.56}{-6.02}{2} & {$\pm$}2.11 & \numpmRF{+6.74}{-6.31}{2} & \numpmRF{+3.76}{-3.29}{2} & \numpmRF{+9.21}{-10.47}{2} \\
325 & [305, 350] & 29.39 & {$\pm$}2.79 & \numpmRF{+2.66}{-2.96}{2} & {$\pm$}2.55 & \numpmRF{+4.55}{-4.22}{2} & \numpmRF{+2.44}{-2.13}{2} & \numpmRF{+6.93}{-6.74}{2} \\
350 & [325, 370] & 20.22 & {$\pm$}1.77 & \numpmRF{+0.39}{-2.21}{2} & {$\pm$}0.56 & \numpmRF{+2.98}{-2.80}{2} & \numpmRF{+1.81}{-1.49}{2} & \numpmRF{+3.97}{-4.29}{2} \\
375 & [345, 395] & 12.57 & {$\pm$}1.12 & \numpmRF{+0.90}{-0.65}{2} & {$\pm$}0.70 & \numpmRF{+1.95}{-1.81}{2} & \numpmRF{+1.24}{-0.93}{2} & \numpmRF{+2.81}{-2.51}{2} \\
400 & [375, 420] & 8.05 & {$\pm$}0.74 & \numpmRF{+0.63}{-1.01}{2} & {$\pm$}0.14 & \numpmRF{+1.22}{-1.13}{2} & \numpmRF{+0.95}{-0.62}{2} & \numpmRF{+1.83}{-1.80}{2} \\
\bottomrule
\end{tabular}
\caption{Breakdown of uncertainties for the signal in $SR\equiv D2$.}
\label{tab:syst:signal}
\end{center}
\end{table}


==> tab-xsect-signal.tex <==
%%------------------------------  
\begin{table}[!ht]
\begin{center}\renewcommand\arraystretch{1.6}
\footnotesize
\begin{tabular}{c|c|c|l|l}
\toprule
$\mstop$ [GeV] & $N_{\rm raw} $ & $\epsilon_{\rm gen}$ & $\sigma_{\rm prod.}~[{\rm pb}]$ & $\int \lumi dt~[\invfb]$
\\
\midrule
\multicolumn{5}{c}{Events with no generator filter$^{(a)}$} \\
\midrule
100 & 300000 & $1$ & $5.6 \times 10^{2}$ & $0.54$ \\
125 & 300000 & $1$ & $2 \times 10^{2}$ & $1.5$ \\
150 & 299000 & $1$ & $80$ & $3.7$ \\
175 & 200000 & $1$ & $37$ & $5.5$ \\
200 & 200000 & $1$ & $19$ & $11$ \\
225 & 200000 & $1$ & $9.9$ & $20$ \\
250 & 200000 & $1$ & $5.6$ & $36$ \\
275 & 100000 & $1$ & $3.3$ & $30$ \\
300 & 100000 & $1$ & $2$ & $50$ \\
325 & 100000 & $1$ & $1.2$ & $80$ \\
350 & 100000 & $1$ & $0.81$ & $1.2 \times 10^{2}$ \\
375 & 100000 & $1$ & $0.53$ & $1.9 \times 10^{2}$ \\
400 & 100000 & $1$ & $0.36$ & $2.8 \times 10^{2}$ \\
\midrule
\multicolumn{5}{c}{Extra events with generator leading truth jet $p_T$-filter$^{(b)}$} \\
\multicolumn{5}{c}{(anti-$k_t$ truth, $R=0.4$, $p_T>100\gev$)} \\
\midrule
100 & 200000 & $0.17$ & $5.6 \times 10^{2}$ & $2.1$ \\
125 & 200000 & $0.32$ & $2 \times 10^{2}$ & $3.2$ \\
150 & 200000 & $0.49$ & $80$ & $5.1$ \\
175 & 100000 & $0.65$ & $37$ & $4.2$ \\
200 & 100000 & $0.79$ & $19$ & $6.8$ \\
225 & 100000 & $0.88$ & $9.9$ & $11$ \\
250 & 100000 & $0.93$ & $5.6$ & $19$ \\
\bottomrule
\end{tabular}
\caption{Number of generated MC events ($N_{\rm raw}$), generator filter efficiency ($\epsilon_{\rm gen}$), production cross-section ($\sigma_{\rm prod.}$), and equivalent luminosity ($\int \lumi dt$) for the stop signal processes. Note that the extra events were generated to improve the statistics in the signal region, in particular for low mass stops. The events with and without the generator $p_T$-filter were combined using a weighted average: $\langle\epsilon_{\rm gen}\rangle = \left(N^{(a)}_{\rm raw} + N^{(b)}_{\rm raw}\right) / \left(N^{(a)}_{\rm raw}/\epsilon^{(a)}_{\rm gen} + N^{(b)}_{\rm raw}/\epsilon^{(b)}_{\rm gen}\right) $. }
%$\langle\epsilon_{\rm gen.}\rangle = \left(N^{(a)}_{\rm raw.}/\epsilon^{(a)}_{\rm gen.} + N^{(b)}_{\rm raw.}/\epsilon^{(b)}_{\rm gen.}\right) / \left(N^{(a)}_{\rm raw.} + N^{(b)}_{\rm raw.}\right)$.}

\label{tab:aux-sig-cross-section}
\end{center}
\end{table}
%%------------------------------  

